Classical Codes and Chiral CFTs at Higher Genus

Higher genus modular invariance of two-dimensional conformal field theories (CFTs) is a largely unexplored area. In this paper, we derive explicit expressions for the higher genus partition functions of a specific class of CFTs: code CFTs, which are constructed using classical error-correcting codes. In this setting, the $\mathrm{Sp}(2g,\mathbb Z)$ modular transformations of genus $g$ Riemann surfaces can be recast as a simple set of linear maps acting on $2^g$ polynomial variables, which comprise an object called the code enumerator polynomial. The CFT partition function is directly related to the enumerator polynomial, meaning that solutions of the linear constraints from modular invariance immediately give a set of seemingly consistent partition functions at a given genus. We then find that higher genus constraints, plus consistency under degeneration limits of the Riemann surface, greatly reduces the number of possible code CFTs. This work provides a step towards a full understanding of the constraints from higher genus modular invariance on 2d CFTs.

==> backups/conclusion_back_up_1.tex <==

In this paper we have spelled out the relation between higher weight enumerator polynomials of classical error-correcting codes and chiral CFT partition functions at higher genus. Given a code $\mathcal C$, the corresponding genus $g$ partition function $Z^{(g)}$ can be found by following two steps. First, due to Construction A, the code defined a modular covariant function on the Siegel upper half-plane $\IM \Omega\succ0$ given by evaluating the genus $g$ enumerator polynomial $W_{\mathcal C}$ in terms of theta constants, \eqref{eq:thetamapdef}. Second, the genus $g$ partition function is given by the modular invariant $W_{\mathcal C}(\vartheta_i(\Omega))/F_g(\Omega)^{c}$. Schematically, we can write
\begin{equation}
    \text{Code $\mathcal C$} \longrightarrow W_{\mathcal C}^{(g)}(\vartheta_i(\Omega)) \longrightarrow Z^{(g)}(\Omega)=\frac{W_{\mathcal C}^{(g)}(\vartheta_i(\Omega))}{F_g(\Omega)^c}.
\end{equation}

The two ingredients in our relation have previously been considered separately. The first step defines a map $\Th:R_g\to M_g$ from the ring of homogeneous polynomials in $2^g$ variables satisfying the generalized McWilliams identities to the ring of genus $g$ Siegel modular forms. Since $R_g$ has an algebraically simple structure, the $\Th$ map has been useful in characterizing the ring $M_g$ of Siegel modular forms \cite{Runge1996,Oura2008} \JH{More references}. The second step implies that at a given central charge $c$, partition functions of chiral CFTs must be a linear combination of Siegel modular forms of degree $c/2$, which was exploited in \cite{Gaberdiel:2010jf,Keller:2017iql} to find bases for chiral CFT partition functions at low values of $c$. 

For genus $g\leqslant3$, we have shown that it is possible to go directly from an enumerator polynomial, i.e. polynomial in $2^g$ variables $x_i$ satisfying the generalized MacWilliams identities, to a genus $g$ CFT partition function, without invoking the complete description of the ring of Siegel modular forms. The only non-trivial information about modular forms entering the discussion is the relation $\Th(j^{(3)})=0$ at genus $3$, which could have been found empirically by evaluating the involved theta constants numerically or in a series expansion. By comparing with the path through Siegel modular forms, we get as a byproduct of our approach expressions for the Siegel modular forms in polynomial basis, agreeing with previous results by Runge \cite{Runge1996}. We give some of these expressions in appendix~\ref{app:modularformsincodebasis}.

At genus $g\geqslant4$, as we discussed in section~\ref{sec:beyond}, the situation is much more complicated. The $\Th$ map, constistuting the essential part in the first step, is known to be non-surjective starting from genus 5 (surjectivity at genus 4 is an open question). Moreover, the second step becomes non-trivial since the moduli space $\mathcal M_g$ of genus $g$ Riemann surfaces is no longer dense in (the quotient of) the Siegel upper half-plane, potentially allowing for ``exotic'' partition functions that do not lift to Siegel modular forms. Hence we restricted the main computations in section~\ref{sec:enumeration} to $g\leqslant 3$.

The main motivation for our work was some observations made in \cite{Dymarsky:2020qom}, which studied the relation between codes and CFT partition functions at genus $1$. By solving the MacWilliams identities over polynomials with integer coefficients, some solutions were found that did not correspond to partition functions of known CFTs. For instance, at $c=24$, 190 solutions were found, while there are only nine known codes at this value of $c$. Working only at genus 1, there is no way of ruling out the ``fake'' CFTs -- in fact any positive linear combination of two real CFTs with integer coefficients will satisfy all constraints at genus 1. In section~\ref{sec:enumeration}, we saw that imposing that the genus 1 partition function must descend from the factorization of partition functions at genus 2 and 3 reduces the number of solutions to 29 and 21 respectively.\footnote{In fact, for $g\leqslant6$, there are linear relations between the enumerator polynomials of the nine codes at $c=24$ \cite{Oura2008}. \JH{Can we speculate about the implications of this results?}}

A limitation of our approach is that the expressions involved when searching for integer solutions of the McWilliams identities become unmanageable as $c$ and $g$ increase. The parametrization by Runge \cite{Runge1996} in terms of ``admissible polynomials'' reduces the size of the involved expressions but this merely delays the problem to slightly larger $c$. As we discussed in section~\ref{subsubsec:findinglatticethetas}, it may be possible to improve the algorithms to incorporate the positive geometry imposed by the positivity conditions. We also noted that our algorithm, imposing positivity of the enumerator polynomial, did not capture all lattice CFTs, since some lattices correspond to enumerator polynomails with negative coefficients, see table~\ref{tab:c=24}. Naturally, this means that our method may also rule out more exotic CFTs. It would therefore be desirable to find a way to implement positivity on the level of conformal data (non-negative integer multiplicities of states, and non-negative squared OPE coefficients), as was done at genus $g\leqslant 2$ in \cite{Keller:2017iql}, see also \cite{Cho:2017fzo,Cardy:2017qhl}.

Finally, we would like to discuss the relation between quantum error-correcting codes, Lorentzian lattices and (non-chiral) CFTs at higher genus, something we hope to return to in future work \cite{Future}. The enumerator polynomial of a quantum error-correcting code at genus $g$ is a polynomial in $2^{g-1}(2^g+1)=3,10,36,\ldots$ variables, which under a suitable generalisation of the $\Th$ map correspond to certain real-analytic theta series.
%Again, the genus $1$ case was considered in \cite{Dymarsky:2020qom}, and ``fake CFTs'' arise already at $c=3$, being ``averages'' of real CFTs. We note, however, that this type of averaging is not the same as in the recent interesting developments relating averages of Narain moduli space to theories of quantum gravity \cite{Afkhami-Jeddi:2020ezh,Maloney:2020nni}. In that case, one considers a continuous average was over Narain moduli space of theories on a specific lattice; in the case of ``fake CFTs,'' the average is over a discrete set of theories corresponding to different lattices. 







%%%%%%%%%%%%%%%%%%%%%% Intro backup




Two-dimension conformal field theories are among the best understood quantum field theories, and yet a lot remains unknown. This is especially true for theories with central charge $c> 1$, where unitarity allows for infinite dimensional representations of the Virasoro algebras. The resulting theories are, in general, much more complicated than those theories with $c<1$. One powerful method for studying 2d conformal field theories (CFTs) is the modular bootstrap \cite{Hellerman:2009bu}, which constrains the torus partition function based on the requirement that it be invariant under the $\mathrm{PSL}(2,\mathbb{Z})$ group of modular transformations. The constraints from genus 1 modular invariance have been used to derive universal bounds on the spectrum, including bounds on the dimension gap, twist gap, and operator degeneracies \cite{Cardy:1986ie,Hellerman:2010qd, Keller:2012mr, Friedan:2013cba, Qualls:2013eha, Kim:2015oca, Collier:2016cls, Benjamin:2016fhe, Dyer:2017rul, Anous:2018hjh, Bae:2018qym, Lin:2019kpn, Afkhami-Jeddi:2019zci, Hartman:2019pcd}.
\begin{table}
\centering
\caption{Dictionary relating Error correcting codes and CFTs.}\label{tab:genus1highergenus}
{\renewcommand{\arraystretch}{1.75}
\begin{tabular}{>{\RaggedRight\arraybackslash}p{4.5cm}>{\RaggedRight\arraybackslash}p{4.5cm}>{\RaggedRight\arraybackslash}p{4.5cm}}
Codes & Lattice & CFT's
\\\hline
n (dimension of code), & n (dimension of \mathbb{R}^n), & $\frac{c}{2}$ (c is the central charge)
\\\hline
W_\mathcal{C}, & \Theta_{\Lambda(\mathcal{C})}(\Omega), & Z_g
\\\hline
HD (Hamming distance), & Shortest vector , & Spectral  gap 
\\ \hline
Doubly-even self dual, & Even self-du
\end{tabular}
}
\end{table}

The torus partition function fully specifies the spectrum of the theory, but contains no information about the dynamics, \emph{i.e.}\ the OPE coefficients. For this reason, it is unable to completely define a theory. This is clear from cases where different theories have the same genus 1 partition function, the most famous of which arise from Milnor's example of two isospectral self-dual even lattices in 16 dimensions, which define isospectral CFTs with $c = 16$ \cite{Milnor}. Perhaps more surprisingly, there exist examples of modular invariant functions, decomposable in Virasoro characters with non-negative integer multiplicities, which do not correspond to any known CFT; for an example in the non-chiral case, see section~6 of \cite{Dymarsky:2020qom}. The dynamical information can, in principle, be addressed using the full conformal bootstrap method \cite{Rattazzi:2008pe} to bound sphere four-point functions using crossing symmetry, however these constraints are not easily combined with those of modular invariance. %Furthermore, in the holographic approach to studying AdS${}_3$. This has been particularly relevant in recent work on 3d quantum gravity from an average over Narain moduli space; see \cite{Maloney:2020nni, Afkhami-Jeddi:2020ezh}.

The higher-genus partition functions might offer a way to bound the spectrum and OPE coefficients at the same time. It was argued in \cite{Moore:1988qv} that consistency of 2d CFTs with crossing symmetry and modular invariance implies that the theory can be consistently defined on Riemann surfaces of any genus. The same Riemann surface can be obtained by sewing together simple three-holed spheres in different ways -- higher-genus consistency essentially means that the resulting partition function must not depend on the sewing procedure. This leads to the requirement that the partition function is invariant under the full genus-$g$ modular group $\mathrm{Sp}(2g, \mathbb{Z})$. Unlike the torus partition function, the higher-genus partition functions do contain information about the OPE coefficients. This leads to the natural question: to what degree does the set of higher-genus partition functions characterize a 2d CFT? This view that a 2d CFT may be defined by its vacuum amplitudes for all genera, originally advanced in \cite{Friedan:1986ua}, has been addressed more recently in \cite{Gaberdiel:2009rd, Gaberdiel:2010jf}. Other recent interest in deriving universal bounds from higher-genus modular invariance include \cite{Keller:2017iql, Cho:2017fzo, Cardy:2017qhl}. 

In this paper, we will use 2d CFTs defined by error-correcting codes (ECCs) to study higher-genus modular invariance. Error-correcting codes are reviewed at more length in section~\ref{sec:review}, but simply speaking, a $c$-dimensional code is a collection of binary vectors of length $c$. These vectors can be visualized as a vertices on a unit hypercube. Importantly, this means that an error correcting code be used to define a lattice, simply by identifying the vectors in the code with the unit cell of the lattice (this is the so-called ``Construction A'', of Leech and Sloane \cite{Leech1993}).





There are two main reason


of this paper will be to consider higher-genus modular invariance in a very particular, concrete setting. These are the code CFTs, reviewed in section~\ref{sec:review} and defined as follows: Given a classical error correcting code (ECC), there is a systematic way of defining a lattice. If the ECC is doubly-even and self-dual, then the lattice will be even and self-dual. Compactifying $c$ free bosons on an $c$-dimensional even self-dual Euclidean lattice results in a chiral CFT with central charge $c$ \cite{cmp/1104286871}, a chiral version of the construction of Narain CFTs \cite{Narain:1985jj,Narain:1986am}. This correspondence leads to a number of non-trivial relations between quantities derived from the CFT and those derived from the ECC. The most important one for our purposes is the relation between the CFT torus partition function and the code's enumerator polynomial. From the code perspective, the enumerator polynomial is a simple object which counts the lengths of the elements of the code. The relationship between code enumerator polynomials and partition functions has been known for genus 1 for a long time \cite{Dolan:1989kf} \cite{Dolan:1994st}. Recently it has been shown \cite{Dymarsky:2020bps, Dymarsky:2020qom} that the correspondence between classical codes and chiral CFTs has a generalization to quantum error correcting codes and full non-chiral CFTs, also that limited to genus 1.

In this paper, we will show how the relation between partition functions and error correcting codes extends to higher genus. This requires the introduction of the ``higher-weight'' enumerator polynomial, known in the literature on ECCs at least as early as \cite{MacWilliams1972}. The weight $g$ enumerator polynomial generalizes the weight 1 enumerator polynomial from a sum over codewords to a sum over $g$-tuples of codewords. We show that the weight $g$ enumerator polynomial is related to the genus-$g$ partition function. As a result, higher-genus modular invariance implies constraints on the allowed higher-weight enumerator polynomials. Such constraints are have been long known in the math literature \cite{MacWilliams1972}, but the connection to higher-genus constraints on CFTs has, as far as we know, not yet been worked out.

Code CFTs give a particularly simple setup to study higher-genus modular invariance because that the modular transformations can be recast as \emph{linear} transformations on the higher-weight enumerator polynomial. This means that we will actually be able to \emph{solve} the constraints of higher-genus modular invariance for the special case where the partition is given by a code enumerator polynomial. By further requiring that all of the coefficients of the polynomial are positive integers, we can list every partition function which could possible derive from an error-correcting code. In cases where we know the set of codes (such as for $c = 24$) this list includes the enumerator polynomials of all real codes, plus a number of ``fake'' enumerator polynomials which are known not to correspond to codes. Whether or not they correspond to CFTs at all is an open question.

We impose a further constraint, called ``factorization limits'': when the higher-genus Riemann surface degenerates into two lower-genus Riemann surfaces connected by an infinitely thin, long tube, then the higher-genus partition function must factorize into the products of lower-genus partition functions. This constraint greatly reduces the number of possible partition functions; most higher-genus partition functions do not factorize correctly, and most lower-genus partition functions do not arise from higher-genus partition functions via the factorization limit. Such partition functions \emph{cannot} possibly arise from error-correcting codes via Construction A.\footnote{However, our approach cannot rule out the possibility that the genus one ``fake'' partition functions corresponds to CFTs which have partition functions at higher genus that cannot be constructed from an enumerator polynomial with positive integer coefficients.} We show this explicitly for genus 1, 2, and 3. We speculate that performing the algorithm laid out here for arbitrarily high genus would eliminate every partition function except those arising from ECCs. 

For genus 1, 2 and 3 and any central charge $c$, we find that our results have an interesting geometrical structure. The requirement that the enumerator polynomials have positive integer coefficients means that the allowed enumerator polynomials form a discrete set indexed by a few coefficients which obey simple linear inequalities. More specifically, these coefficients live in a polytope whose dimension is equal to one less than the number of independent Siegel modular forms with weight $c/2$. This dimension grows as the genus grows, but the higher-genus polytope can always be projected to the lower-genus space, and its projection must be inside the polytope defined by the lower-genus constraints. This means that each genus gives stricter constraints than the previous one, at least for $g = 1$, $g = 2$, and $g = 3$.

%We find that many many of these fake partition functions do not arise from higher genus partition functions via these factorization limits. This gives an independent proof that these fake partition functions \emph{cannot} possibly arise from error-correcting codes via Construction A -- in principle this could be used to constrain the number of error correcting codes of a given size.\footnote{However, our approach cannot rule out the possibility that the genus one ``fake'' partition functions corresponds to CFTs which have partition functions at higher genus that cannot be constructed from an enumerator polynomial with positive integer coefficients.} Pushing this technique to high enough genus must uniquely fix the set of invariant polynomials to be those which arise from error-correcting codes. We see this concretely for the codes with $c = 16$, which give rise to the isospectral theories discussed before. These codes have the same weight 1 and weight 2 enumerator polynomials, but different weight 3 polynomials.\footnote{In fact, these codes give rise to a pair of theories which cannot be distinguished from the partition function until genus \emph{five}. This stems from the complicated degeneracies that arise in the map between enumerator polynomials and partition functions at $g \geq 3$. See section~\ref{subsec:maths} for a discussion.}

%An interesting consequence of the higher-genus correspondence between ECCS and CFTs is that code CFTs are completely characterized by their higher-weight enumerator polynomials. This follows from the fact that an error-correcting code of dimension $k$ is uniquely determined by its weight-$(k-1)$ enumerator polynomial \cite{Runge1996}.\footnote{The dimension of the code equals the central charge of the corresponding CFT.} Fully specifying the code specifies the lattice on which the CFT lives. Each lattice vector determines both the scaling dimension (by its length) and the conserved charges (by its components) of the state corresponding to the vector. This, in turn, fixes the operator algebra. Note that this argument relies heavily on the fact that lattice theories are free, so their dynamics are entirely determined by their quantum numbers (an analogous argument applies to Narain theories, which are theories of free bosons compactified on even self-dual \emph{Lorentzian} lattices). However, it is not clear if this means that they can be characterized by their higher-genus partition functions because, as we shall see, the map from enumerator polynomials to partition functions is not invertible for genus $g \geqslant 3$.

% Another interesting byproduct of our work is a set of explicit expressions for genus 2 and 3 Siegel modular forms in terms of the polynomials of theta constants, on which modular transformations act as linear maps. These expressions facilitate easy manipulation of the forms -- for example, it is obvious in our basis if a form is a product of two other forms. The relationship between error-correcting codes and modular forms at higher genus was already known in \cite{Runge1996}, where it was shown that the space higher-weight enumerator polynomials derived from self-dual codes maps directly onto the space of Siegel modular forms (of degree divisible by four).\footnote{At genus 1, the relations imposed by modular invariance are equivalent to the well-known relations on code enumerator polynomials that lead to Gleason's theorem.} Furthermore, some interesting recent work \cite{Gaberdiel:2010jf,Keller:2017iql} has exploited the fact that partition functions of meromorphic chiral CFTs can be parametrized by Siegel modular forms to bound the space of possible partition functions at genus 2 \cite{Gaberdiel:2010jf,Keller:2017iql}. In part, this work will combine and extend these approaches to constrain the space of code CFTs. We believe that our approach would be particularly interesting in the case of quantum error-correcting codes, which correspond to non-chiral CFTs and where the theory of modular forms is much less developed. This will be explored in a future paper \cite{Future}.

The outline of the paper is as follows. In section \ref{sec:review}, we review the correspondence described above in the case of chiral CFTs at genus 1. In section \ref{sec:Higher Genus}, we show how to extend the correspondence between codes and CFTs to higher genus, focusing on the higher-weight enumerator polynomial and how it is constrained by the symmetries and factorization properties required by the CFT. We also comment on some issues related to genus $g>3$. In section \ref{sec:enumeration}, we show explicitly how to use these constraints to determine every allowed enumerator polynomial for a given genus $g$ and dimension $c$. We do this for $c$ up to $48$ for genus $2$ and $c$ up to $24$ for genus 3. We show where the real ECCs lie in the space of allowed enumerator polynomials. We also use our results to fix the genus 2 Siegel modular forms in terms of the polynomial variables of ECCs.



